Enhanced 3DMM Attribute Control via Synthetic Dataset Creation Pipeline

While facial attribute manipulation of 2D images via Generative Adversarial Networks (GANs) has become common in computer vision and graphics due to its many practical uses, research on 3D attribute manipulation is relatively undeveloped. Existing 3D attribute manipulation methods are limited because the same semantic changes are applied to every 3D face. The key challenge for developing better 3D attribute control methods is the lack of paired training data in which one attribute is changed while other attributes are held fixed -- e.g., a pair of 3D faces where one is male and the other is female but all other attributes, such as race and expression, are the same. To overcome this challenge, we design a novel pipeline for generating paired 3D faces by harnessing the power of GANs. On top of this pipeline, we then propose an enhanced non-linear 3D conditional attribute controller that increases the precision and diversity of 3D attribute control compared to existing methods. We demonstrate the validity of our dataset creation pipeline and the superior performance of our conditional attribute controller via quantitative and qualitative evaluations.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> sections/note.tex <==
% 1. Real vs. Generated (measure: FID)

%     Baseline model
    
%         GT dist. 300W-3D (ex. 남자 분포)
        
%         Comparisons
%         Real - 300W-3D (모든 데이터 써서 gender 방향 추출)
%             %  (- FFHQ)
             
%         Generated
%              - synthetic (synthetic 써서 gender방향 추출)
        
%         (각 방향 벡터를 GT에 적용해서 FID비교)
        
%     Objective: 
%     Desired result: "comparable"
%     우리 pipeline이 제대로 만들어졌다 (synthetic데이터 쓸만함).
    
    
    


2. Baseline vs. Conditional Attribute Controller 
    
    a. training in synthetic, testing in synthetic (measure: Euclidean distance)
    
    % GT dist. 300W-3D
    % b. (ours): training in synthetic,
    %   (baseline): training in synthetic
       
    %   testing in real(300W-3D) (measure: FID (이미지에서))
       

    Objective:
    Desire result: "win"
    
    우리가 제안한 conditional attribute controller가 기존 global attribute transformation에 비해 우수한 성능을 보임.

3. Real Baseline vs. Synthetic AC.
    a. (ours): training in synthetic,
       (baseline): training in real (CelebA or FFHQ)
       
       testing in real(CelebA or FFHQ) (measure: FID )
    
    
    Objective:
    Desire result: "win"
    
    우리가 제안한 entire frameworks including the data creation pipeline and conditional attribute controller가 기존 global attribute transformation에 비해 우수한 성능을 보임.
    
    
    
    
layer1 synthetic L2 : file dir (models_l2), fold 존재  
    B: norecon
    B: norecon_nores
    A: norecon_noscore

layer1 norecon L file dir (models_new2), fold 없음
    B: CelebA Mahalanobis distance
    
    
% noscore
# norecon (B)
# pred_param = src_SET_param + pred_trans_param

# norecon_nores (B)
# pred_param = pred_trans_param

# norecon_noscore (A)
pred_param = src_SET_param + trg_distance*pred_trans_param

%${\hat{p}}$ cos similarity
% x N => off-diagonal mean




%baseline:
synthetic에서 nores 돌리기


쪼끄만 figure
(synthetic)
L2 (정답 같이 있는거)

paramter 변화에 따른 방향의 차이
output direction 출력

FFHQ에서 모든 attribute에 대해 우리 모델 결과 뽑기





Supplemantary material:
- StyleUV 활용한 attribute 변환
- Score 변환에 따른 attribute 별 변화 (1줄 당 각 attribute, 박스로 인풋 표현)
- random sample () 한 p에서 가는거 2개 attribute만 
